On superconvergence of Runge-Kutta convolution quadrature for the wave equation

The semidiscretization of a sound soft scattering problem modelled by the wave equation is analyzed. The spatial treatment is done by integral equation methods. Two temporal discretizations based on Runge-Kutta convolution quadrature are compared: one relies on the incoming wave as input data and the other one is based on its temporal derivative. The convergence rate of the latter is shown to be higher than previously established in the literature. Numerical results indicate sharpness of the analysis. The proof hinges on a novel estimate on the Dirichlet-to-Impedance map for certain Helmholtz problems. Namely, the frequency dependence can be lowered by one power of $\abs{s}$(up to a logarithmic term for polygonal domains) compared to the Dirichlet-to-Neumann map.

==> figures/conv_mod.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=6]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{loglogaxis}[
    width=\textwidth, height=7cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$n$,
    ylabel=$H^{-1/2}$-error,
    legend style={legend pos=south west},
    %legend style={legend pos=outer south, legend cell align=left},
    %legend style={at={(0,-0.22)},anchor=north west,legend cell align=left},
%    xtick= ,
    x tick label style={/pgf/number format/1000 sep=\,}   
    ]



    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau5_mod.csv};    


    \addplot+[solid,mark=triangle,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau3_mod.csv};    

    
    \addplot [black,dashed ] expression [domain=16:128, samples=15] { 3E07*x^(-7)}
    node [pos=0.9,inner sep=0pt, anchor=south west] {{\small $\bigO(k^{7})$}};

    \addplot [black,dashed ] expression [domain=64:1024, samples=15] { 3E07*x^(-5)}
    node [pos=0.9,inner sep=0pt, anchor=south west] {{\small $\bigO(k^{5})$}};


    %\addplot [black,dashed ] expression [domain=32:2048, samples=15] { 5*x^(-1)} node [pos=0.8,inner sep=2pt, anchor=south west] {{\small $\bigO(\Delta t)$}};

    
  \end{loglogaxis} 
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../super"
%%% End:


==> figures/conv_r3.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=6]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{loglogaxis}[
    width=6.2cm, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$n\sim 1/k$,
    ylabel=$H^{-1/2}$-error,
    legend style={legend pos=south west},
    %legend style={legend pos=outer south, legend cell align=left},
    %legend style={at={(0,-0.22)},anchor=north west,legend cell align=left},
%    xtick= ,
    x tick label style={/pgf/number format/1000 sep=\,}   
    ]



    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau3_std.csv};    


    \addplot+[solid,mark=triangle,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau3_mod.csv};    

    
    \addplot [black,dashed ] expression [domain=64:4048, samples=15] { 3E04*x^(-3)}
    node [pos=0.7,inner sep=0pt, anchor=south west] {{\small $\bigO(k^{3})$}};

    \addplot [black,dashed ] expression [domain=64:1624, samples=15] { 3E07*x^(-5)}
    node [pos=1.0,inner sep=0pt, anchor=south west] {{\small $\bigO(k^{5})$}};

    \legend{standard, differentiated}

    %\addplot [black,dashed ] expression [domain=32:2048, samples=15] { 5*x^(-1)} node [pos=0.8,inner sep=2pt, anchor=south west] {{\small $\bigO(\Delta t)$}};

    
  \end{loglogaxis} 
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../super"
%%% End:


==> figures/conv_r5.tex <==
\pgfplotsset{
  log x ticks with no point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[precision=0]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=6]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{loglogaxis}[
    width=6.2cm, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$n\sim 1/k$,
    ylabel=$H^{-1/2}$-error,
    legend style={legend pos=south west},
    %legend style={legend pos=outer south, legend cell align=left},
    %legend style={at={(0,-0.22)},anchor=north west,legend cell align=left},
%    xtick= ,
    %x tick label style={/pgf/number format/1000 sep=\,},
%    x tick label style=
    x tick label style={log x ticks with no point},
    xtick = {4, 8,16,32,64,128,256}
    ]



    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau5_standard.csv};    


    \addplot+[solid,mark=triangle,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=n,
    y=e,
    col sep=comma
    ]{figures/data/error_new_radau5_modified.csv};    

    
    \addplot [black,dashed ] expression [domain=10:200, samples=15] { 2E05*x^(-5)}
    node [pos=0.7,inner sep=0pt, anchor=south west] {{\small $\bigO(k^{5})$}};

    \addplot [black,dashed ] expression [domain=10:100, samples=15] { 2E06*x^(-7)}
    node [pos=0.6,inner sep=0pt, anchor=north east] {{\small $\bigO(k^{7})$}};


    \legend{standard, differentiated}
    %\addplot [black,dashed ] expression [domain=32:2048, samples=15] { 5*x^(-1)} node [pos=0.8,inner sep=2pt, anchor=south west] {{\small $\bigO(\Delta t)$}};

    
  \end{loglogaxis} 
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../super"
%%% End:


==> figures/corner.tex <==
%\documentclass{standalone}% For the example only, any class will do

%\usepackage{tikz}
%\usetikzlibrary{positioning}% To get more advances positioning options
%\usetikzlibrary{arrows}% To get more arrow heads

%\begin{document}
\begin{tikzpicture}[scale=1.4]
 
  %\fill[blue!20] ( -2, 0) to[out=25,in=190] (-1,0.125) to[out=-180+190,in=180] (0,0)
  % -- (1,1) -- (0,1) to[out=190,in=0] (-1,0.125+1) to[out=0+180,in=190+180] ( -2, 0+1);
  % \draw[very thick] ( -2, 0) to[out=25,in=190] (-1,0.125) to[out=-180+190,in=180] (0,0);

  \fill[green!20] ( -2, 0) -- (0,0)
   -- (1,1) -- (0,1) to[out=190,in=0] (-1,0.125+1) to[out=0+180,in=190+180] ( -2, 0+1);
   \draw[very thick] ( -2, 0) -- (0,0);

   
   
   %\fill [red!20](0,0) to[out=-100,in=90+15] (0.25, -1 ) to[out=90+15-180,in=90] (0.5,-2)   
   %-- (0.5+1,-2) to[out=90+15,in=180+90] (0.25+1, -1) to[out=180-100,in=180+90+15]  (1,1) -- (0,0);
   %\draw [very thick] (0,0) to[out=-100,in=90+15] (0.25, -1 ) to[out=90+15-180,in=90] (0.5,-2) ;

   \fill [red!20,pattern=crosshatch  dots,pattern color=red!40](0,0) -- (0.5,-2)
   -- (0.5+1,-2) to[out=90+15,in=180+90] (0.25+1, -1) to[out=180-100,in=180+90+15]  (1,1) -- (0,0);
   \draw [very thick] (0,0) --  (0.5,-2) ;

   
   \draw[thick] (0,0) -- (1.5,1.5) node[below] {$\Gamma_j'$};

   \draw[dashed] (0,0) -- (1.7,0);
   \draw[dashed] (0,0) -- (-0.4,1.7);


   \fill (0,0) circle (0.05);
   \node (V) at (-0.25,-0.25)  {$A_{j}$};
   \node[below]  at (-1.5,0.0) {$\Gamma_{j}$};
   \node[right]  at (-0.15,-1.5) {$\Gamma_{j+1}$};

   \node at (-1,0.6) {$\Omega_{j}$};
   \node at (0.8,-0.7) {$\Omega_{j+1}$};

   \draw[dashed] ($(0,0) + (-75:1.4)$) arc (-75:180:1.4);
   \node at (1.5,0.4) {$S_{\omega}$};

   \node at (0,-2.26) {}; %%only here to give same size as domain.tex
    
\end{tikzpicture}
%\end{document}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> figures/domain.tex <==
% \documentclass{standalone}% For the example only, any class will do

% \usepackage{tikz}
% \usetikzlibrary{positioning}% To get more advances positioning options
% \usetikzlibrary{arrows}% To get more arrow heads

% \usepackage{tkz-euclide}
% \usetkzobj{all}

% \begin{document}

%\begin{tikzpicture}[scale=1.3]
\begin{tikzpicture}[scale=1.0]

  \clip(-3,-3.15) rectangle (3,2.5);
  %\draw[thick] (-3,0) -- (-1,2) -- (2,1) -- (3,-1) -- (2,-3) -- (0,-1) -- (-2,-3) -- cycle;

  \coordinate (B1) at (-3,0);
  \coordinate (B2) at (-1,2);
  \coordinate (B3) at (2,1);
  \coordinate (B4) at (3,-1);
  \coordinate (B5) at (2,-3);
  \coordinate (B6) at (0,-1);
  \coordinate (B7) at (-2,-3);

  \draw[thick] (B1) 
  \foreach \x in {2,...,7}
    { -- (B\x)  }%
  -- cycle;
  

  \tkzDefLine[bisector](B1,B2,B3);
  \tkzGetPoint{a1};
  \tkzDefPointBy[homothety=center B2 ratio .15](a1)   \tkzGetPoint{a11}
  \draw[dashed] (B2) -- (a11);
   
  
  \tkzDefLine[bisector](B2,B3,B4);
  \tkzGetPoint{a2};
  \tkzDefPointBy[homothety=center B3 ratio .15](a2)   \tkzGetPoint{a21}
  \draw[dashed] (B3) -- (a21);
  
  \tkzDefLine[bisector](B3,B4,B5);
  \tkzGetPoint{a3};
  \tkzDefPointBy[homothety=center B4 ratio .15](a3)   \tkzGetPoint{a31}
  \draw[dashed] (B4) -- (a31);
  
  
  \tkzDefLine[bisector](B4,B5,B6);
  \tkzGetPoint{a4};
  \tkzDefPointBy[homothety=center B5 ratio .23](a4)   \tkzGetPoint{a41}
  \draw[dashed] (B5) -- (a41);

  
  
  \tkzDefLine[bisector](B7,B6,B5);
  \tkzGetPoint{a5};
  \tkzDefPointBy[homothety=center B6 ratio -.125](a5)   \tkzGetPoint{a51}
  \draw[dashed] (B6) -- (a51);
  
  %\tkzDrawLine[add=0.1 and -1,dashed ](B6,a5);

  \tkzDefLine[bisector](B6,B7,B1);
  \tkzGetPoint{a6};
  \tkzDefPointBy[homothety=center B7 ratio .2](a6)   \tkzGetPoint{a61}
  \draw[dashed] (B7) -- (a61);
  

  \tkzDefLine[bisector](B7,B1,B2);
  \tkzGetPoint{a7};
  \tkzDefPointBy[homothety=center B1 ratio .15](a7)   \tkzGetPoint{a71}
  \draw[dashed] (B1) -- (a71);
  
  
  \draw[dashed,blue] plot [smooth cycle] coordinates {  (a11)  (a21)  (a31)  (a41)  (a51)  (a61)  (a71) };


  %\tkzDrawBisector[dashed,thin](B6,B7,B1);
  %\tkzDrawBisector[dashed,thin](B7,B1,B2);


  \fill[dashed,opacity=0.2,blue] ($(B1) + (-72:1)$) arc (-72:45:1.) -- (B1);
  \fill[dashed,opacity=0.2,blue] ($(B2) + (-134:0.9)$) arc (-134:-18:0.9) -- (B2);
  \fill[dashed,opacity=0.2,blue] ($(B3) + (162:1)$) arc (162:298:1) -- (B3);
  \fill[dashed,opacity=0.2,blue] ($(B4) + (115:0.7)$) arc (115:244:0.7) -- (B4);
  \fill[dashed,opacity=0.2,blue] ($(B5) + (64:1.1)$) arc (64:136:1.1) -- (B5);
  \fill[dashed,opacity=0.2,blue] ($(B6) + (-45:0.8)$) arc (-45:225:0.8) -- (B6);
  \fill[dashed,opacity=0.2,blue] ($(B7) + (44:1.2)$) arc (44:110:1.2) -- (B7);

  \node (l1) at (-0.9,-1.6) {$\Omega_{j}$};
  \node (l2) at (1.0,-1.6) {$\Omega_{j+1}$};

  \node (l3) at (1.0,-2.5) {$\Gamma_{j+1}$};

  \node (l4) at (-1.0,-2.4) {$\Gamma_{j}$};
  
  \fill (B6) circle  (0.05);
  \node[right](LV1) at (B6) {$A_j$};

  \fill (B5) circle  (0.05);
  \node[right](LV2) at (B5) {$A_{j+1}$};
  \fill (B7) circle  (0.05);
  \node[right](LV3) at (B7) {$A_{j-1}$};
  
\end{tikzpicture}

%\end{document}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

